Big Data Analytics for QoS Prediction Through Probabilistic Model Checking

As competitiveness increases, being able to guaranting QoS of delivered services is key for business success. It is thus of paramount importance the ability to continuously monitor the workflow providing a service and to timely recognize breaches in the agreed QoS level. The ideal condition would be the possibility to anticipate, thus predict, a breach and operate to avoid it, or at least to mitigate its effects. In this paper we propose a model checking based approach to predict QoS of a formally described process. The continous model checking is enabled by the usage of a parametrized model of the monitored system, where the actual value of parameters is continuously evaluated and updated by means of big data tools. The paper also describes a prototype implementation of the approach and shows its usage in a case study.

==> section4-casestudy_old.tex <==
\section{The Smart Grid Case Study}
\label{sec:casestudy}
The proposed QoS Prediction approach has been validated with respect to a Smart Grid (SG) case study. 

SG is the integration of the IT infrastructure into a traditional power grid in order to continuously exchange and process information to better control the production, consumption and distribution of electricity. For this purpose Smart Meters (SMs) devices are used to measure variations of electric parameters (e.g. voltage, power, etc.) and send such data to a computational environment which, in turn, analyse and monitor it in a real-time fashion.


In this case study, our tool performs the remote monitoring on behalf of an Energy Distributor (ED) which purchases electric power from Energy Producers (EPs) and retails it to Energy Consumers (ECs). The primary goal of the ED is to balance the purchased electric power with respect to the variations of power demand. 
\\
\textbf{The SG Model.}
For the sake of simplicity we have built a basic model which represents an ED, EP (or aggregated values of many EPs) and EC (or aggregated values of many ECs) as a three-queue system networked as in fig. \ref{fig:sg-model}. 
%
\begin{figure*}[!htb]
\centering
\includegraphics[scale=0.6]{sg-model_ver2}
\caption{Network queuing system model}
\label{fig:sg-model}    
\end{figure*}
%
Each queue is a discrete representation of the real-valued KPI to be modelled. 
The PRISM-based model we define implements the queues $ED_Q$, $EP_Q$, and $EC_Q$ with queue length and transition rates as parameters. 
Furthermore, the sets $A_V$, $C_V$, $I_V$ are arranged as follows:
\[ \footnotesize
\begin{split}
	A_V &= \{d_e : d_e\ge adm_{min}\; \text{and}\; d_e\le adm_{max}\} \\
	C_V &= \{d_e : -cri_{min}\le d_e< adm_{min}\}\; \cup \\ 
		& \quad \cup \{d_e: adm_{max}< d_e \le cri_{max}\} \\
	I_V &= \{d_e : d_e<-cri_{min}\; \text{or}\; d_e>cri_{max}\}
\end{split}
\]
%
where $adm_{max}$, $adm_{min}$ and $cri_{min}$ and $cri_{max}$ represent the minimum and maximum thresholds of the admissible and critical value sets.
\\ 
\\
\textbf{Parameters Updating.}
In the queuing model the queue length and the transition rate are updated as follows.
Two thresholds are set on both queue edges so that if the current state goes below the first or up the second, the queue length is doubled or halved respectively. 
As for the updating of the transition rate, an Exponential Weighted Moving Average (EWMA) is applied on the first difference of the time series %\footnote{Such computation is applied on both time series, i.e. the power production and consumption} 
under analysis. Thus, let $Y = y_1,y_2,...$ a time series, we compute the transition rate $\rho$ as follows:
\begin{equation} \label{eq:update}
\rho' = 
\end{equation}
in which the initial value of $\rho$ is set to $0$. The \ref{eq:update} is used for both the increment ($\mu_t$) and the decrement rate ($\lambda_t$).
\newline\newline
\textbf{QoS Data Extraction.}
To tackle the Big Data issue, our architecture takes advantage of a Complex Event Processing (CEP) which could be performed on any data-intensive distributed framework (e.g. Hadoop). Such combination allows to extract, process and deliver (complex) data in real-time, empowering the QoS monitoring and prediction phases.
Following our case study, we show an example of a complex event to derive the \textit{balance indicator} (BI) from the basic SmartMeterMeasureEvent originating from the Smart Meters of EPs and ECs: 
\begin{verbatim}
insert into BalanceIndicatorEvent
select (EP.measure - EC.measure) as index 
from EP.SmartMeterMeasureEvent as EP, 
	 EC.SmartMeterMeasureEvent as EC,

select "range_i"
from BalanceIndicatorEvent
where index index >= I_min and <= I_max
\end{verbatim}

The first query compute the BI and create the event \verb|BalanceIndicatorEvent|. The second query is a template used by our QoS Monitoring tool to generate the actual queries. They are used to classify at which range the index belongs to. Based on this data, the QoS Analyser component compute the transition rate from one range to another to be fed the PRISM model. 
On the other side, a temporal-based query is used for a real-time anomalous detection:
\begin{verbatim}
select measure, "CriticalValueMsg" 
from EP1.SmartMeterEvent.win:time(15 min)
where measure < BASE_PROD
\end{verbatim}

In this case we take advantage of the temporal-based capability of the CEP language. The select deliver a \verb|CriticalValueMsg| message based on the fact that a specific energy producer (EP1 in the example) is gone underproduction. The message is delivered to the QoS Monitoring which in turn perform the associated action, e.g. notify ED.
%
\newline\newline
\textbf{Quality Constraints to be Monitored.}
Briefly we report only two types of QCs: the first is a safety property (neither \textit{within} nor \textit{along} operator specified) which assesses if the predicted violation probability in the next 15 minutes is more than 10\%.
\begin{equation} \label{prop:1}
\footnotesize
	\text{\bf eval}(\mathcal{P}_{\ge 0.1}[F_{\le 30} \verb|"violState"|]) = \verb|false|
\end{equation}

The second QC guarantees to be notified if the probability of incurring in a violation state in the next 30 minutes is greater than 0.05 for two subsequent times (considering a measurement events every 15 minutes). 

\begin{equation} \label{prop:2}
\footnotesize
	\text{\bf eval}(\mathcal{P}_{=?}[F_{\le 30} \verb|"violState"|]) \le 0.05\; \text{\bf within}\; 30m\; 
\end{equation}

\subsection{Validation}
\label{sec:valid}
%
\begin{table*}[!htb] \footnotesize
\centering
\begin{tabular}{c|ll|lll}
\hline
\bf Queue length  & \bf \#States & \bf \#Trans & \bf BM time (s) & \bf MC time (s) & \bf Tot. time (s)\\ \hline 
% 10 & 2040 & 9336 & 0.03  & 0.08 & 0.11 \\ 
 20 & 13280 & 63476 & 0.15 & 0.38 & 0.53 \\ 
% 30 & 41720 & 202416 & 0.35 & 2.44 & 2.79 \\ 
 40 & 95360 & 466156 & 0.81 & 8.37 &  9.18\\ 
% 50 & 182300 & 894696 & 3.17 & 27.01 &  30.18\\ 
 60 & 310240 & 1528036 & 7.75 & 52.51 & 60.27 \\ 
% 70 & 487480 & 2406176 & 13.39 & 135.49 & 148.88 \\ 
 80 & 721920 & 3569116 & 20.53 & 197.11 & 217.64 \\ 
% 90 & 1021560 & 5056856  & 27.53  & 355.29 & 382.82 \\ 
 100 & 1394400 & 6909396 & 42.80 & 492.28 & 535.089 \\ 
\hline 
\end{tabular} 
\caption{Queues length, model size, and execution time}
\label{tab:modelsize-time}
\end{table*}

In our scenario we assume a balance range of 800 Mega Watt (MW), i.e. $[min_b=-400,max_b=400]$, and we firstly evaluate how much time the QoS prediction phase takes with respect to different model size (Table \ref{tab:modelsize-time}). 
The table also reports the size of the model in terms of number of states and transitions. As expected by using a model-ckeching technique, the time is exponential against the model size. However, as the last row shows, we can also observe that even in case of millions ($10^6$) of states and transitions - that means a fine-grained discretisation - the total time is less than 9 minutes, hence still comparable with the updating rate usually considered for SGs. 

We have selected a queue length of 40 - i.e. a unit increment/decrement of the queue correspond to a 20MW of balance variation - and set these thresholds: $adm_{min} = -200$, $adm_{max} = 200$, $cri_{min} = -380$, $cri_{max} = 380$. Our tests are based on property \ref{prop:2} evaluated by simulating three different scenarios: %variation in the current balance state.
\begin{description}
\item[Scenario A:] EPs inject in the grid as much energy as ECs need (balanced case).\\
\item[Scenario B:] ECs request less than EPs produce (overproduction).\\
\item[Scenario C:] The energy consumption request rises twice compared with the production rate (imbalanced condition).
\end{description}

\begin{figure*}[!htbp]
\centering
\includegraphics[scale=0.5]{violation-vs-balance-state2}
\caption{Violation Probability (queue length=40)}
\label{fig:viol-balance}     
\end{figure*}
Fig. \ref{fig:viol-balance} plots the violation probability estimated for such scenarios.
For scenario A the violation probability varies in a symmetrical fashion around the balance point (i.e. queue length 20).  
The scenario B exhibits a higher probability in all the overproduction states (i.e. queue length less than the balance point), and a lower one for a large number of states representing the power grid overload (i.e. queue length greater than the balance point). 
This characteristic is emphasised in the third simulation which represents the imbalanced (overloaded in this case) scenario. In addition, we notice how in such anomalous conditions all minimum values of violation probability are higher than the other two scenarios.
